How do Software Ecosystems Co-Evolve? A view from OpenStack and beyond

Much research that analyzes the evolution of a software ecosystem is confined to its own boundaries. Evidence shows, however, that software ecosystems co-evolve independently with other software ecosystems. In other words, understanding the evolution of a software ecosystem requires an especially astute awareness of its competitive landscape and much consideration for other software ecosystems in related markets. A software ecosystem does not evolve in insulation but with other software ecosystems. In this research, we analyzed the OpenStack software ecosystem with a focal perspective that attempted to understand its evolution as a function of other software ecosystems. We attempted to understand and explain the evolution of OpenStack in relation to other software ecosystems in the cloud computing market. Our findings add to theoretical knowledge in software ecosystems by identifying and discussing seven different mechanisms by which software ecosystems mutually influence each other: sedimentation and embeddedness of business relationships, strategic management of the portfolio of business relationships, firms values and reputation as a partner, core technological architecture, design of the APIs, competitive replication of functionality and multi-homing. Research addressing the evolution of software ecosystem should, therefore, acknowledge that software ecosystems entangle with other software ecosystems in multiple ways, even with competing ones. A rigorous analysis of the evolution of a software ecosystem should not be solely confined to its inner boundaries.

==> wp-template.config.tex <==
\RequirePackage{etoolbox}


\RequirePackage{xcolor}
\definecolor{bmcblue}{rgb}{0,0.2,0.4}
\definecolor{joseViolet2016}{rgb}{0.44,0.16,0.39}


\definecolor{docheadcolor}{rgb}{0.44,0.16,0.39}



\newcommand{\wpAuthCorrespondant}{{\color{joseViolet2016}{$\star$}}}
\newcommand{\wpAuthSymbFirst}{{\color{blue}$\vardiamondsuit$}}
\newcommand{\wpAuthSymbSecond}{{\color{blue}$\clubsuit$}}
\newcommand{\wpAuthSymbThird}{{\color{blue}$\spadesuit$}}





==> wp-template.head.tex <==
% Calls some bmc package !! Not sure what it does 
\usepackage[bmc]{bmcart-biblio}




\usepackage[utf8]{inputenc} %unicode support
%\usepackage[applemac]{inputenc} %applemac support if unicode package fails
%\usepackage[latin1]{inputenc} %UNIX support if unicode package fails

\usepackage[english]{babel} % Language hyphenation and typographical rules


%From http://www.latextemplates.com/template/journal-article
\usepackage{blindtext} % Package to generate dummy text throughout this template 



% Sets helvetical font for captions and headers 
\usepackage[scaled=.90]{helvet}


% text main font
\usepackage[sc]{mathpazo} % Use the Palatino font
% Better  T1 (extended characters support, better PDF support, widely used).
\usepackage[T1]{fontenc} % Use 8-bit encoding that has 256 glyphs
\linespread{1.05} % Line spacing - Palatino needs more space between lines



% Advanced tweack with pdflatex 
% See http://www.khirevich.com/latex/microtype/ for explanation
\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
% activate={true,nocompatibility} - activate protrusion and expansion
% final - enable microtype; use "draft" to disable
% tracking=true, kerning=true, spacing=true - activate these techniques
% factor=1100 - add 10% to the protrusion amount (default is 1000)
% stretch=10, shrink=10 - reduce stretchability/shrinkability (default is 20/20)



\usepackage{enumitem} % Customized lists
\setlist[itemize]{noitemsep} % Make itemize lists more compact

% For the support of entrance epigraphs 
\usepackage{epigraph}


\usepackage{lettrine} % The lettrine is the first enlarged letter at the beginning of the text



\usepackage{abstract} % Allows abstract customization
\renewcommand{\abstractnamefont}{\normalfont\bfseries} % Set the "Abstract" text to bold
\renewcommand{\abstracttextfont}{\normalfont\small\itshape} % Set the abstract itself to small italic text


\usepackage{titlesec} % Allows customization of titles
\renewcommand\thesection{\Roman{section}} % Roman numerals for the sections
\renewcommand\thesubsection{\roman{subsection}} % roman numerals for subsections
\titleformat{\section}[block]{\large\centering\bfseries}{\thesection.}{1em}{\vspace{0.3em}} % Change the look of the section titles
%\titleformat{\subsection}[block]{\large}{\thesubsection.}{1em}{} % Change the look of the section titles
\titleformat{\subsection}[block]{\normalfont\large\bfseries}{}{0.0em}{\vspace{0.15em}} % Change the look of the section titles

% To resize table
\usepackage{adjustbox}

% Fancytables 
\usepackage{booktabs}

\usepackage{array,tabularx} % To have the table fill out the page

% For table notes 
\usepackage[flushleft]{threeparttable}


% Changes the font of table enviroment.
\makeatletter
\appto\@floatboxreset{%
  \ifx\@captype\andy@table
    \normalfont
    %\rmfamily
  \fi
}
\def\andy@table{table}
\makeatother


% Enable simple arithmetic in LaTeX commands
\usepackage{calc}

% for repeated footnotes 
\usepackage{footmisc}

% For symbols 
\usepackage{stix}

% Footnotes with long url need special attention 
% See https://tex.stackexchange.com/questions/23394/url-linebreak-in-footnote
% And https://groups.google.com/forum/#!topic/pandoc-discuss/Ttvfpz7zTCY
\usepackage[hyphens,spaces,obeyspaces]{url}
\def\UrlBreaks{\do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\%\do\;\do\>\do\]%
\do\)\do\,\do\?\do\'\do\+\do\=\do\#\do\-}%
\Urlmuskip=0mu plus 1mu %





